The pinched Veronese has no Koszul filtration

In this paper we prove that the pinched Veronese subalgebra $k [x^3,x^2y,xy^2,x^2z,xz^2,y^3,y^2z,yz^2,z^3] \subset k[x,y,z]$ has no Koszul filtration regardless of the field $k$, despite it being a Koszul algebra. We do this by showing that no ideal $(f,g)$ minimally generated by two linear forms can belong to a Koszul filtration. By the definition of a Koszul filtration this, in turn, implies that no Koszul filtration can exist.

==> chapters/lastlemma.tex <==

\begin{tikzcd}
	{ } & PV & PV & {PV/(f,g)} & 0
	\arrow[from=1-1, to=1-2]
	\arrow["{d_2}", from=1-2, to=1-3]
	\arrow["{d_1}", from=1-3, to=1-4]
	\arrow["{d_0}", from=1-4, to=1-5]
\end{tikzcd}

$$d_0=(f,g)$$
$$d_1=\begin{pmatrix}
    g_0x^2&g_0y^2&g_0z^2&g_0Q\\
    f_0x^2&f_0y^2&f_0z^2&f_0Q
\end{pmatrix}$$
 $$d_2=\text{non-linear}$$
